Deep Smoothing of the Implied Volatility Surface

We present a neural network (NN) approach to fit and predict implied volatility surfaces (IVSs). Atypically to standard NN applications, financial industry practitioners use such models equally to replicate market prices and to value other financial instruments. In other words, low training losses are as important as generalization capabilities. Importantly, IVS models need to generate realistic arbitrage-free option prices, meaning that no portfolio can lead to risk-free profits. We propose an approach guaranteeing the absence of arbitrage opportunities by penalizing the loss using soft constraints. Furthermore, our method can be combined with standard IVS models in quantitative finance, thus providing a NN-based correction when such models fail at replicating observed market prices. This lets practitioners use our approach as a plug-in on top of classical methods. Empirical results show that this approach is particularly useful when only sparse or erroneous data are available. We also quantify the uncertainty of the model predictions in regions with few or no observations. We further explore how deeper NNs improve over shallower ones, as well as other properties of the network architecture. We benchmark our method against standard IVS models. By evaluating our method on both training sets, and testing sets, namely, we highlight both their capacity to reproduce observed prices and predict new ones.

==> sections/discussion.tex <==
\section{Discussion} \label{sec:discuss}

\subsection{Broader Impact}

\fbox{TODO:} some ideas:
\begin{itemize}
\item options can be used as insurance to protect against losses
\item measures can be built from the options market on the financial health and expectations of the markets, e.g.\ VIX index
\item model interpretability is important for financial implication, and particularly financial regulation. Hence controlled asymptotic make the application more meaningful.
\end{itemize}

%\subsection{Extensions}
%
%\fbox{TODO:} maybe for the conclusion?
%
%The presented approach focuses on a single stock and observations at a single time because this already represents a challenging and relevant practical problem.
%Still, we discuss how one could approach the modeling of multiple stocks, and the IVS at multiple time points.
%
%\textbf{Multi-asset.}
%It is straightforward to extend the current approach to create a model for multiple IVSs.
%Indeed, one may consider a model taking as input an input categorical variable that will the volatility surface.
%This approach would allow to transfer reuse and transfer features learned from on surface to another, which could be highly beneficial in situations where few observations are available for IVS.
%This advantage typically comes at the cost of building and training a deeper and larger NN for a joint model than for individual models.
%Note that, additional non-arbitrage constraints may have to be imposed in the specific case of implied volatility surfaces for currency pairs.
%
%\textbf{Multi-day.}
%Modeling the IVS at multiple time points could be useful to transfer information forward from the past, which may be allows to build a more resilient image of the IVS a given time point.
%This may be achieved in different ways.
%For example, the parameters $\theta$ of the previous model could be used as initial values for the model to be newly fitted.
%Alternatively, one may think of propagating forward in time a latent factor as performed in recurrent neural networks.
%
%Another application could the construction of a generative model for future IVSs which could be used for risk-management, for example.
%Such a generative model would be required to simulate entire IVSs given present and past values.
%Our approach could be used in combination with a generative module to guarantee that the fake IVSs are sensible.

==> sections/emp_ana.tex <==
\section{Empirical analysis}\label{sec:emp}

\fbox{TODO:}
In practice, we linearly interpolated and extrapolated $\watm$. 

\input{tables/appli_stats}

In this section, we apply our approach to modeling implied volatility surfaces extracted from S\&P500 options prices between.
More specifically, we use a dataset containing the price of all options traded during January 2018, namely 61812 contracts, and \Cref{tab:appli_stats} displays daily summary statistics.

We perform the following exercise for each day in the sample.
First, we split the daily sample into a training and a testing set.
Second, we fit the model on the training set and evaluate its performance on the testing set.
As described in~\Cref{tab:intraextra}, we use two different configurations for training and testing.
In the interpolation setting, for each maturity, we randomly select half of the contracts.
As such, we also sample options that are far out or in the money for training, and the testing error represents the approximation error for the range of moneyness that are actually observed.
In the extrapolation setting, for each maturity, we select 70\% of the contract that have an absolute Call option Delta in the range $[0.02,0.98]$, see the Appendix~B.2.
This second filter is equivalent to selecting approximately 50\% of all the contracts but with more observation around the money.
Thus, we do not select options that are far out or in the money for training, and the testing error measures how well our model extrapolates.
Finally, we again use the three set of conditions described in~\Cref{tab:conditions} to study how the arbitrage-related penalties affect the results.

\begin{table}
%\begin{wraptable}{r}{0.6\textwidth}
\caption{Settings for the training and testing sets.\label{tab:intraextra}}
\centering
\begin{tabular}{ l c c   }
  \hline
    & Call Delta & Train/(Train + Test) \\
\hline
   Interpolation & 0--1 & 0.5 \\
\hline
   Extrapolation & 0.02--0.98 & $\approx$ 0.5 \\
\hline
\end{tabular}
%\end{wraptable}
\end{table}

In~\Cref{tab:appli_loss}, we present our results.
First, we describe the RMSE and MAPE.
As expected, training errors are generally below testing errors.
Somewhat surprisingly, extrapolation errors are most of the time smaller than interpolation errors.
This may be because the surface is highly non-linear around the money, i.e.\ around $k=0$, while the surface wings tend to be more linear.
While MAPE errors might seem large, it should be noted that, for some contracts, the implied volatility is extremely small and thus even tiny deviations significantly impact this error measure.
Interestingly, we see that the second condition (i.e., strong enforcement of the no-arbitrage constraints) also leads to the smallest interpolation and extrapolation errors.
Furthermore, comparing the first and third conditions, we see that even a mild no-arbitrage constraint provides improvements over simply trying to minimize the RMSE and MAPE.
Regarding CAL and BUT, we see that the models resulting from condition 1 and 2 are essentially arbitrage-free.
As for the model resulting from no enforcement of the constraints (i.e., condition 3), it provides calendar-spread arbitrage opportunities both in interpolation and extrapolation, as well as butterfly arbitrage opportunities in extrapolation.

Time-series of the daily losses can be found in Appendix~C.3.
\vspace{-0.2cm}

\input{tables/appli_loss}




==> sections/num_exp.tex <==
\section{Numerical experiments} \label{sec:num}

\fbox{TODO:}
\begin{itemize}
\item move feature engineering to the appendix
\item discuss parameter initialization
\item simplify training routine?
\end{itemize}

%% Optimization and default initialization
\textbf{Evaluation metric and experimental setup.} 
The method of the previous section is implemented using tensorflow \cite{abadi2016tensorflow} and available in the supplementary material.
The total loss $\Lcal(\theta)$ is minimized with the Adam Optimization Algorithm \citep{kingma2014adam}, and the parameters initialized randomly with uniform random variables on the compact $[-1, 1]$ with the exception of $b_{n+1}$ which is initialized at $\log(20\%)$.
As adaptive learning rate and early stopping have shown to significantly improve training \citep{haykin2009neural, hagan1994training, sutskever2013importance, caruana2001overfitting, prechelt1998early, hinton2015distilling}, we follow this approach.
Starting with a learning rate of $0.01$, we let it decrease by a factor $2$ on plateaus of length $500$ epochs when the total loss was not improved by more than $1\%$.
The learning routine stops if $\Lcal(\theta)$ has not improved by $1\%$ over $2000$ epochs, and restarts using the initial learning rate until $10000$ total epochs have been reached or until the total loss \eqref{eq:loss} is below $1\%$.

\textbf{Convergence.}
To explain the large number of epochs, note that the signal-to-noise ratio for empirical volatility surfaces is generally large, and overfitting is seldom the main concern in this context.
Furthermore, because datasets contain at most a few thousand samples at most and only two features (moneyness and time-to-maturity), we are not using minibatch.

\textbf{Feature engineering.} We observed that the inclusion of features inversely proportional to the time to maturity helped to calibrate the ANN models with fewer layers and neurons.
We conjecture that this is because the implied volatility surface tends to sharply increase with $\lvert k \rvert$ at short horizons while being more flat at longer horizons.
Therefore, we include an initial static layer $f_0$ defined by
\begin{equation}\label{eq:feateng}
X = f_0(k,\tau) = \left(k, \, \tau, \, k \tau^{-0.5}, \, k \tau^{-0.95} \right).
\end{equation}
Note that conditions~\ref{cons:posi}--\ref{cons:vmat} remain satisfied with these features, and that the total variance remains asymptotically linear in $k$. 
The input dimension is now $\nc{1}=4$.

\textbf{Calibration models and Baselines.}
To study the properties of our approach in a controlled setting, we create two synthetic datasets using the Heston and Bates models, see Appendix~B.1.
We use the following vector of moneyness values $[0.3, 0.4, 0.6, 0.8, 0.9, 0.95, 0.975, 1, 1.025, 1.05, 1.1, 1.2, 1.3, 1.5, 1.75, 2, 2.5, 3]$, and maturities 
of half a week, one, two and three weeks, one to twelve months, eighteen months and two years.

Parameters common to the Heston and Bates model are 
$V_0 = 0.10^2$,
$\theta = 0.25^2$,
$\rho = -0.75$,
$\kappa =  0.5$, and
$\sigma = 1$.
Jump parameters specific to the Bates model are 
$\lambda = 0.1$,
$\beta = -0.05$, and
$\alpha = 0.15$.
We also set the interest rate and dividend yield to zero.

\textbf{Model flexibility check.}
We first show that, as expected, the ANN model can reproduce any surface given enough parameters.
In Appendix~C.1 we show that the ANN model with four layers, 20 neurons per layer, and without arbitrage constraints is flexible enough to fit synthetic data and market data.
In the following we will therefore use this configuration as an upper bound in terms of flexibility, focusing on the impact of arbitrage constraints and architecture choice, i.e.\ number of layers and neurons.


\textbf{Losses convergence.}
We study the loss and speed of convergence for different configurations.
We calibrate models with two and four hidden layers, five and twenty neurons per layers, and using the ReLu activation function.
In~\Cref{tab:conditions}, we summarize the different conditions for the arbitrage penalties: 
$\lambda_1$ (respectively $\lambda_2$) is the weight corresponding to~\eqref{eq:losscal} (respectively~\eqref{eq:lossbut}).
The first condition represents a vanilla case, where the fit and arbitrage related losses have an equal weight.
In the second condition, absence of arbitrage is enforced more strictly by increasing the weight of the penalties.
In the third condition, we perform an ablation study to see how well we do when absence of arbitrage is not enforced.

\begin{table}
%\begin{wraptable}{r}{0.35\textwidth}
\caption{Settings for the penalties\label{tab:conditions}}
\centering
  \begin{tabular}{ c  c c }
\toprule
  Condition & $\lambda_1$ & $\lambda_2$ \\
  \hline
  1 & 1 & 1 \\
  2 & 10 & 10 \\
  3 & 0 & 0 \\
\bottomrule
\end{tabular}
%\end{wraptable}
\end{table}

\Cref{fig:conv_loss} displays the different loss terms in~\eqref{eq:loss}.
First, we see that increasing the number of layers or of neurons per layers generally decreases the RMSE and MAPE.
Second, we observe that, when the number of layers is smaller, increasing the neurons per layer without enforcing more strictly the constraints can generate arbitrage opportunities.
But such opportunities disappear when absence of arbitrage is given a higher weight.

\Cref{fig:conv_iter} displays the total number of iteration necessary before the calibration algorithm stops.
As expected, increasing the number of layers or of neurons per layers leads to slower convergence.
Interestingly, enforcing absence of arbitrage more strictly decreases the number of iterations required to converge.

Results for the Heston model can be found in Appendix~C.2.

\begin{figure}
%\begin{wrapfigure}{l}{0.6\textwidth}
\centering
\includegraphics[width=0.6\textwidth]{figures/numexp_convergence_loss_bates.pdf}
\caption{Losses for different combination of number of layers and neurons per layer. Synthetic data is generated from the Bates model.\label{fig:conv_loss}}
%\end{wrapfigure}
\end{figure}

\begin{figure}
%\begin{wrapfigure}{r}{0.6\textwidth}
\centering
\includegraphics[width=0.6\textwidth]{figures/numexp_convergence_iter_bates.pdf}
\caption{Number of iterations before the calibration stops for different combination of number of layers and neurons per layer. Synthetic data is generated from the Bates model.\label{fig:conv_iter}}
%\end{wrapfigure}
\end{figure}

\textbf{Smoothing behaviors.}
A major challenge is the extrapolation of the implied volatility surface to unobserved data points.
Flexible non-parametric methods typically fail as they lack the guidance of a parametric model.
In \Cref{fig:smoothing} we calibrate ANN models with different loss terms and parameters initialization on a subsample of 100 options with narrow moneyness on the synthetic Bates data. 
The three models fit the train set almost perfectly.
Yet, we see that the ANN without arbitrage losses, $\lambda_1=\lambda_2=0$, fails extrapolate in a nonsensical way.
On the other hand the arbitrage-free model with $\lambda_1=\lambda_2=10$ behaves very smoothly.
The last model is initialized with the weights of an ANN model fitted to a Bates model itself fitted on the train set, see Appendix~B.3.
It is furthermore penalized so that its weights remain close to its initialization weights with $\lambda_3=1$.
This confirms that a regularized learning can produce an extrapolation mimicking the Bates model, with most notable differences in this example for the positive log-moneynesses.


\begin{figure}
  \centering
  \input{figures/smoothing}
  \vspace{-0.8cm}
\caption{Extrapolation with different loss specification and weights initialization.\label{fig:smoothing}}
\end{figure}




%% no time
%%\textbf{Soft versus hard constraints.}





==> tables/appli_loss.tex <==
\begin{table}[!h]

\caption{Mean loss (with standard deviation).
    All numbers are multiplied by 100.
    \label{tab:appli_loss}}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llllllll}
\toprule
\multicolumn{2}{c}{ } & \multicolumn{2}{c}{Condition 1} & \multicolumn{2}{c}{Condition 2} & \multicolumn{2}{c}{Condition 3} \\
\cmidrule(l{3pt}r{3pt}){3-4} \cmidrule(l{3pt}r{3pt}){5-6} \cmidrule(l{3pt}r{3pt}){7-8}
 &  & Interpolation & Extrapolation & Interpolation & Extrapolation & Interpolation & Extrapolation\\
\midrule
 & train & 3.12 (3.04) & 4.79 (5.82) & 2.47 (2.98) & 1.56 (3.58) & 5.46 (1.91) & 8.1 (5.7)\\
\cmidrule{2-8}
\multirow[t]{-2}{*}{\raggedright\arraybackslash RMSE} & test & 9.48 (7.52) & 4.87 (5.91) & 7.66 (6.95) & 1.55 (3.47) & 14.27 (4.67) & 8.2 (5.75)\\
\cmidrule{1-8}
 & train & 16.04 (15.67) & 16.39 (19.88) & 12.81 (15.46) & 5.42 (12.43) & 27.96 (10.09) & 27.66 (19.43)\\
\cmidrule{2-8}
\multirow[t]{-2}{*}{\raggedright\arraybackslash MAPE} & test & 26.4 (22.65) & 16.66 (20.11) & 21.61 (21.91) & 5.48 (12.26) & 42.14 (13.54) & 27.76 (19.45)\\
\cmidrule{1-8}
 & train & 0.01 (0.02) & 0.02 (0.03) & 0.03 (0.07) & 0.07 (0.18) & 4.24 (2.75) & 2.39 (1.78)\\
\cmidrule{2-8}
\multirow[t]{-2}{*}{\raggedright\arraybackslash CAL} & test & 0.01 (0.02) & 0.02 (0.03) & 0.03 (0.07) & 0.07 (0.18) & 4.24 (2.75) & 2.39 (1.78)\\
\cmidrule{1-8}
 & train & 0 (0) & 0 (0) & 0 (0) & 0 (0) & 0.86 (2.06) & 3.36 (14.06)\\
\cmidrule{2-8}
\multirow[t]{-2}{*}{\raggedright\arraybackslash BUT} & test & 0 (0) & 0 (0) & 0 (0) & 0 (0) & 0.86 (2.06) & 3.36 (14.06)\\
\bottomrule
\end{tabular}}
\end{table}


==> tables/appli_stats.tex <==
\begin{table}
%\begin{wraptable}{r}{0.75\textwidth}
\caption{\label{tab:appli_stats}Daily statistics for January 2018.}
\centering
\begin{tabular}{lrrrr}
\toprule
 & Mean & Std & Min & Max\\
\midrule
Max moneyness & 1.274 & 0.017 & 1.239 & 1.304\\
Min moneyness & 0.186 & 0.019 & 0.174 & 0.241\\
Number of contracts & 3434.000 & 193.934 & 3063.000 & 3747.000\\
Number of maturities & 30.722 & 0.461 & 30.000 & 31.000\\
\bottomrule
\end{tabular}
%\end{wraptable}
\end{table}
